PDNNet: PDN-Aware GNN-CNN Heterogeneous Network for Dynamic IR Drop Prediction

IR drop on the power delivery network (PDN) is closely related to PDN's configuration and cell current consumption. As the integrated circuit (IC) design is growing larger, dynamic IR drop simulation becomes computationally unaffordable and machine learning based IR drop prediction has been explored as a promising solution. Although CNN-based methods have been adapted to IR drop prediction task in several works, the shortcomings of overlooking PDN configuration is non-negligible. In this paper, we consider not only how to properly represent cell-PDN relation, but also how to model IR drop following its physical nature in the feature aggregation procedure. Thus, we propose a novel graph structure, PDNGraph, to unify the representations of the PDN structure and the fine-grained cell-PDN relation. We further propose a dual-branch heterogeneous network, PDNNet, incorporating two parallel GNN-CNN branches to favorably capture the above features during the learning process. Several key designs are presented to make the dynamic IR drop prediction highly effective and interpretable. We are the first work to apply graph structure to deep-learning based dynamic IR drop prediction method. Experiments show that PDNNet outperforms the state-of-the-art CNN-based methods and achieves 545x speedup compared to the commercial tool, which demonstrates the superiority of our method.

==> Doc/answer.tex <==
{
\onecolumn
\normalsize

\ \\
\textbf{Responses to the reviewers}


We would like to firstly thank all the reviewers for their comments and our responses are as follows.

\ \\
\textbf{Reviewer 1}
\begin{description}\itemsep.8em

\item[R1C1]
\textbf{
It is difficult to understand how PDNGraph is constructed based on a given PDN. For example, how to decide the ``node" of a PDN? Seems it depends on the 'uniform grid' defined by the authors, but is the grid division methodology also dependent on the PDN topology?
}
\item[R1A1]
% Thank you for the comment. We regard the circuit layout as a checkerboard, where each grid covers multiple cells and is defined as the “node” of our PDNGraph. Since the edge distance implicitly represents the metal resistance and capacitance of the adjacent node, we opt for the 'uniform grid' to construct the PDNGraph to ensure each edge has consistent attributes. Typically, the grid can be set to any size that affects the computation overhead and IR drop prediction accuracy. To balance the tradeoff between these two aspects, we divide the circuit design in CircuitNet into 256 x 256 grids. It is worth noting that the grid size in our circuit division method is relatively small compared to the pitch of the high-layer power strip in PDN. Thus, our method only considers the pitch of high-power metal in PDN topology and opts for the “uniform grid“ division method.

Thank you for the comment. 
%
In our approach, we regard the circuit layout as a checkerboard, defining each grid that covers multiple cells as a ``node" within our PDNGraph. 
%
The edge distances between nodes implicitly encapsulate the resistance and capacitance characteristics of the metal connecting adjacent nodes. 
%
To ensure uniformity in these attributes, we employ a ``uniform grid" strategy for constructing the PDNGraph, which guarantees consistent edge properties across the graph.
%
Additionally, the grid size is a critical parameter that influences both computational overhead and the accuracy of IR drop predictions. 
%
To balance the tradeoff between these two aspects, we divide the circuit design in CircuitNet into 256 $\times$ 256 grids. 
%
It is important to highlight that the selected grid size is relatively small compared to the pitch of the high-layer power rails in PDNs.
%
Consequently, our division method adopts a ``uniform grid" approach for spatial division. 


\item[R1C2]
\textbf{
For the cell power, are we counting the total power within a grid as the node feature? Then how many features (i.e., C) do we have for each node?
}
\item[R1A2]
% Thank you for the comment. Yes, each cell’s power contributes to the total power in each grid, so we sum the whole power of the cells within the same grid as the node feature in the data processing. We use the power feature extracted from CircuitNet, which follows the PowerNet~\citep{xie_powernet_2020} feature processing protocol. The feature of each node is {Pi, Ps, Psca, Pall, Pt}, which contains 24 channels in total. Specifically, 4 channels for {Pi, Ps, Psca, Pall} and 20 channels for power pattern Pt with different timestamps.

Thank you for your comment. Yes, the total power contribution of each cell within a grid is summed to calculate the overall power, which we then use as the node feature during data processing. These power features are extracted from CircuitNet, following the feature processing protocol established by PowerNet~\citep{xie_powernet_2020}. 
%
Specifically, the feature vector for each node comprises 5 different types of power, Pi, Ps, Psca, Pall, Pt, encompassing a total of 24 channels. 
%
% Here, the first four categories {Pi, Ps, Psca, Pall} are allocated one channel each, while the power pattern Pt is detailed across 20 channels, capturing temporal variations at different timestamps. 
%
Here, 4 channels for {Pi, Ps, Psca, Pall} and 20 channels for power pattern Pt at different timestamps.
%
% This comprehensive feature representation is instrumental in enhancing the accuracy and robustness of our power grid analysis within the PDN framework.


\item[R1C3]
\textbf{
For the current direction, how does each node/grid ``align" with the given PDN? How this ``current direction" is represented in features?
}
\item[R1A3]
% Thank you for the comment. Generally, the current transmits from a high power supply VDD rail to a low redistribution VDD layer (i.e. from M7 to M1). The IR drop gradually increases on the low redistribution layer away from the high-layer VDD due to the resistance that exists on the metal strip.  
% %
% Based on this intuition, we build the directed inter-node edge away from the closest high-layer power rail, which is parallel to the low-redistribution strip direction. 
% %
% This directed graph illustrates the actual current flow direction through PDN structure.
% %
% Note that the 'current direction' is only for edge construction and is not represented in input features.

Thank you for your comment. 
%
Typically, current flows from a high-power supply VDD rail to a lower redistribution VDD layer (e.g. from M7 to M1), and the IR drop increases simultaneously due to the inherent resistance of the metal strips. 
%
% As the current flow away from the high-layer VDD rail on the low redistribution layer,
%
Guided by this intuition, we construct directed inter-node edges emanating from the closest of the high-layer power rail, parallel to the low-redistribution strips. 
%
This orientation of edges in the directed graph effectively represents the actual direction of current flow within the PDN structure.
%
Note that the ``current direction" utilized for edge construction is not contained in the input features, It is solely used to guide the structural configuration of the graph to reflect the actual current flow.

\item[R1C4]
\textbf{
Are CNN and GNN inputs based on the same uniform grids? Are they using the same features? Can the authors summarize both input dimensions (width, height, #nodes, channels/features, etc.)?}
\item[R1A4]
% Thank you for the comment. Yes, the inputs of CNN and GNN branches are shared with the same features and based on the same uniform grids. The input feature dimension is 256 $\times$ 256, 24 channels, and contains 65536 nodes in PDNGraph.

Thank you for the comment. Yes, both the CNN and GNN branches share the same input features, which are based on uniform grids. Specifically, the input feature dimension is configured as 256 × 256, comprising 24 channels and encapsulates a total of 65,536 nodes.

\item[R1C5]
\textbf{
Why conduct the experiments on a mini-dataset with only 80 training samples and 20 testing samples, considering a full dataset is already available? The whole dataset includes 10K samples, which is already a rather small number compared with any regular datasets in computer vision. Please consider using the full dataset, or perhaps at least the full test dataset. Otherwise, the authors may need to elaborate how prohibitive is the actual training cost, and demonstrate that such a mini-dataset is a good/better representative of/than the full dataset.
}

\item[R1A5]
Thank you for the comment. We conducted the ablation study on the whole dataset to verify the key design of our methods. We update our results in the ablation study section. Please refer to \Cref{sec:experiments:ablation} for more details.

\item[R1C6]
\textbf{
For Fig 6, seems MAVIREC is also accurate, it's just their "bias/threshold" is not as good. What about reporting Pear in this figure?
}
\item[R1A6]
Thank you for the comment. We report the evaluation metrics for three figures. For the Pearson metric, the comparison between PDNNet and MAVIREC is (0.9789 \emph{vs} 0.9776, 0.9643 \emph{vs} 0.9776, and 0.9662 \emph{vs} 0.9675). 
%
We also list the values of other metrics in the tables. 
%
PDNNet outperforms MAVIREC among all evaluation metrics in case 1 except $R^2$. In cases 2 and 3, PDNNet exceeds MAVIREC in a portion of the metrics, including NMAE, PSNR, and SSIM. The best scores of the methods are \textbf{highlighted}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/visual_compare_1}
\input{Tables/visual_compare_2}
\input{Tables/visual_compare_3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\item[R1C7]
\textbf{
It is surprising that two channels with exactly the same architecture outperform the simple channel. So what is the difference between dual channels and increasing the number of kernels in a single channel? If there are short-cut structures, increasing kernels in a single channel should also help.
}

\item[R1A7]
Thank you for the comment. The computation formula of convolutional networks is,

\begin{equation*}
H' = \frac{H - K}{S} + 1, 
\end{equation*}
\begin{equation*}
W' = \frac{W - K}{S} + 1,
\end{equation*}
\begin{equation*}
\text{Computation} = H' \times W' \times K \times K \times N \times C.
\end{equation*}
where $H$ and $W$ denote the input feature map height and width, K represents the size of the convolution kernel, the size of the output feature map is $H' \times W'$, the number of convolution kernels is $N$, and the stride is $S$. According to the formula, stacking the same two networks is equivalent to widening the kernel $N$ on a single network. Thus, we conduct extra experiments: expand the kernel to double and fourfold for each GNN and CNN architecture. We compare these wider kernel variants with their dual-channel counterparts. The results are represented as follows:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/wider_network}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We observe that the network with more kernels has similar performance compared with its dual-channel counterpart. 

\end{description}


\ \\
\textbf{Reviewer 2}
\begin{description}\itemsep.8em


\item[R2C1]
\textbf{
Can you explain how the cell attributes are extracted and distributed to node attributes? Are they extracted in CircuitNet?
}
\item[R2A1]
% Thank you for the comment. Yes, each cell’s power contributes to the total power in each grid, so we sum the whole power of the cells within the same grid as the node feature in the data processing. We use the power feature extracted from CircuitNet, which follows the PowerNet~\citep{xie_powernet_2020} feature processing protocol. The feature of each node is {Pi, Ps, Psca, Pall, Pt}, which contains 24 channels in total. Specifically, 4 channels for {Pi, Ps, Psca, Pall} and 20 channels for power pattern Pt with different timestamps.

Thank you for your comment. Yes, the power feature extracted from CircuitNet, follows the feature processing protocol established by PowerNet~\citep{xie_powernet_2020}. The feature vector for each node comprises 5 different types of power, {Pi, Ps, Psca, Pall, Pt}, encompassing 24 total channels. Here, 4 channels for {Pi, Ps, Psca, Pall} and 20 channels for power pattern Pt at different timestamps. All these features are extracted using Voltus, a commercial tool used for power and IR drop analysis. The total power contribution of each cell within a grid is summed to calculate the overall power, which we then use as the node feature during data processing.
%
% Here, the first four categories {Pi, Ps, Psca, Pall} are allocated one channel each, while the power pattern Pt is detailed across 20 channels, capturing temporal variations at different timestamps. 


%
% This comprehensive feature representation is instrumental in enhancing the accuracy and robustness of our power grid analysis within the PDN framework.

\item[R2C2]
\textbf{
Experimental results show good performance, but the 3 correlation scores(Pearson, Spearman, Kendall) are less cared for because they are not sensitive to extreme values, especially in designs with large macros. It is recommended to also include structural similarity and hotspot AUC of PowerNet in table II and IV.
}

\item[R2A2]
Thank you for the suggestion. We add the Structural Similarity Index (SSIM) and Area under Curve of MAVIREC and PowerNet in \Cref{table:main}. Previous Table IV with Mini-CircuitNet result no longer exists as we turn to take the whole dataset to conduct the ablation study.

\item[R2C3]
\textbf{
I'm concerned about the R-square value of MAVIREC in TABLE II, does it indicate divergence in training?
}


\item[R2A3]
Thank you for the suggestion. $R^2$, also known as the coefficient of determination, is a statistical measure that represents how well the data fit the regression model. We present the training loss curve below to show that MAVIREC has reached convergence in the training step. However, we could not determine the divergence in training based on only one metric as eight metrics are shown in \Cref{table:main}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/mavi_loss}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\item[R2C4]
\textbf{
A typo: blank bracket in IV.B "The figures from the left to right columns are macro positions in the floorplan, results from MAVIREC []”
}

\item[R2A4]
Thank you for pointing out the writing issue. We have revised this typo.

\end{description}

\ \\
\textbf{Reviewer 3}
\begin{description}\itemsep.8em

\item[R3C1]
\textbf{
The PDN structure is crucial for accurate IR drop prediction. However, typically the PDN in a design will be fairly regular across the entire layout. Mostly a mesh structure unless some ECO has been done to add more power straps in IR drop critical regions. Typically, the pitch of the power grid is constant for most designs in a specific technology node. So, how much of a role does the GNN play? It would be good to have a motivating example in the early parts of the paper, to show the difference in IR drop for a regular vs. an irregular mesh?
}


\item[R3A1]
% Thank you for your highly valued comments. Typically, the higher IR drop appears where the current flow goes through a long distance from the closet high-layer PDN strip. For the circuit design with a fairly regular mesh, the cell with the same current pattern will have a distinctive IR drop value in different positions of the PDN mesh. Thus, our PDNGraph uses different edge directions between nodes that are determined by the high-layer PDN strip to represent the current flow direction through PDN (details are depicted in \Cref{sec:method:PDNGraph}). Sequentially, our GNN branch transfer features among nodes guided by edge direction to mimic the dynamic current flow in PDN structure.
% %
% This process is similar to the IR drop simulation method and can not be represented by purely CNN-based ones.
% %

% For the PDN mesh with different pitch, we present two pictures to depict the graph construction of regular PDN mesh and irregular one. As we mentioned above, the IR drop value is largely related to the distance to the closet high-layer PDN strip. Hence, the area in a width PDN pitch would have a large IR drop value compared to a narrow PDN pitch under the same current consumption, which is shown in the pictures. 


Thank you for your comments. Typically, a higher IR drop is observed where the current traverses a long distance from the nearest high-layer PDN strip. 
%
In a circuit corporate by a fairly regular mesh, cells with the same current pattern may demonstrate distinct IR drop values at different positions within the PDN mesh. 
%
Consequently, our PDNGraph model employs variable edge directions between nodes, which are determined by the high-layer PDN strip to reflect the current flow direction through PDN, as detailed in \Cref{sec:method:PDNGraph}
. 
%
Subsequently, our GNN branch transfers features among nodes, guided by the edge directions, to mimic the dynamic current flow within the PDN structure.
%
This modeling approach is similar to traditional IR drop simulation methods and addresses limitations inherent in purely CNN-based models, which may not effectively capture the current flow behavior.
%

Regarding variations in PDN mesh pitch, we illustrate the graph construction for both regular and irregular PDN meshes through the two figures below. 
%
As previously noted, the IR drop value is significantly influenced by the footprint to the closest high-layer PDN strip. Therefore, areas within a wider PDN pitch are likely to exhibit higher IR drop values compared to those within a narrower pitch, given identical current consumption. This relationship is visually represented in the figures to enhance understanding of the impact of mesh configuration on IR drop characteristics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irr-re}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\item[R3C2]
\textbf{
How much does the IR drop change for designs with the same current distribution and different power grids? That would show the value of you capturing the PDN topology.
}


\item[R3A2]
% Thank you for the comment. Generally speaking, sparse PDN raises a higher IR drop value compared with dense PDN structures under the same current pattern. However, in dynamic IR drop prediction, the composition of dynamic power includes three parts: internal power, switching power, and leakage power. PDN is generally set up before the routing, which would affect switching power related to the routing solution. Thus, it's hard to make two circuit designs with the same current distribution with different power girds for dynamic IR drop prediction.


Thank you for your comment. Generally speaking, sparse PDN configurations exhibit higher IR drop values compared to denser PDN structures when subjected to identical current patterns. However, the composition of dynamic power includes internal power, switching power, and leakage power all related to dynamic IR drop predicting. Typically, the PDN is established prior to routing, which influences the switching power due to its dependence on the routing solution. Consequently, it becomes challenging to maintain consistent current distribution across two circuits that utilize different power grids in real design flow. We will consider constructing a dataset with a similar power pattern and different PDN structure in our further work.

\item[R3C3]
\textbf{
For designs with extremely irregular (irregular meshes with no fixed pitch across the entire design) PDNs that cannot be represented as images, as in [34], how much does the graph help IR drop?
}


\item[R3A3]
% Thank you for the comment. As we mentioned above, the higher IR drop appears where the current flow goes through a long distance from the closet high-layer PDN strip. Due to the construction process in \Cref{sec:method:PDNGraph}, our PDNGraph uses different edge directions (i.e. away from the closest high-layer power strip) and topology connections between nodes to represent the current flow direction through the PDN structure. Thus, the node near the high-layer PDN can propagate the feature to the node away from the PDN in the message-passing procedure in GNN.
% %
% In an extremely irregular PDN mesh, the node in the center area of a wider PDN pitch gathers more features than the node in a narrow pitch, which can be depreciated as having a higher IR drop probability.
% %
% Hence, our PDNGraph can bridge the fine-grained relationship between cells and PDN topology by leveraging the unique attribute in the graph. PDNGraph is helpful for the GNN branch in PDNNet to mimic the process of the simulation-based IR drop acquiring method, which compensates for the lack of fine-grained PDN topology awareness in CNN-based methods.

Thank you for your comment. As previously mentioned, higher IR drop values occur where the current flows a significant distance from the closest high-layer PDN strip. In alignment with the methodologies outlined in \Cref{sec:method:PDNGraph}, our PDNGraph model employs distinct edge directions, oriented away from the nearest high-layer power strip and builds topology connections between nodes to represent the directional flow of current through the PDN structure. 
%
Consequently, nodes near the high-layer PDN can propagate features to nodes further from the PDN during the message-passing procedure in the GNN.
%
In an extremely irregular PDN mesh, a node situated in the central area of a wider PDN pitch accumulates more features compared to a node within a narrower pitch, suggesting a higher probability of IR drop.
%
Therefore, our PDNGraph effectively bridges the relationships between cells and fine-grained PDN topology by capitalizing on the distinctive attributes embedded within the graph structure. This capability significantly enhances the GNN branch within PDNNet, enabling it to mimic the process employed in simulation-based IR drop acquisition methods. This is particularly advantageous as it compensates for the limitations inherent in CNN-based approaches, which typically lack fine-grained awareness of PDN topology.
%
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irr}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\item[R3C4]
\textbf{
Initially, the authors claim that most prior ML-based techniques for IR drop prediction ignore the PDN structure which is crucial for dynamic IR drop prediction. However, later in the paper, Section IIID points to a prior ML-based work that captures the structure of the PDN. Therefore, Section III D seems out of place in the methods section. This is prior art, and comparisons should be discussed in the introduction. It seems like this discussion is hidden away in the methods, but it's a key discussion that should be brought up early in the paper. The paper misleads at the start that no ML-based prior work has taken PDN topology into account. This is incorrect. However, this is only clarified in Section III D. The differences with respect to [34] should be highlighted at the start. So the contribution of the work is clearly brought out at the start. The key contribution is capturing the PDN topology as a graph and not an image in [34] so that GNN and CNN can be used simultaneously.
}

\item[R3A4]
% Thank you for the comment. We would clarify our point of view that the previous work \citep{static-irdrop} targets static IR drop prediction rather than the dynamic IR drop of our PDNNet. Thus, it’s unnecessary to discuss the method \citep{static-irdrop}  in the introduction section as there are two distinctive targets in ML for EDA. So far, PDNNet is still the first work to capture the fine-grained PDN topology in dynamic IR drop prediction. After comprehensive consideration, we would delete this content to avoid misunderstandings between our method and previous methods.

Thank you for your comment. We wish to clarify that the prior work referenced \citep{static-irdrop} focuses on static IR drop prediction, which contrasts with the dynamic IR drop prediction addressed by our PDNNet. 
%
Thus, it’s unnecessary to discuss the method \citep{static-irdrop}  in the introductory section as there are two distinctive targets in ML for EDA.
%
PDNNet represents the inaugural effort to incorporate fine-grained PDN topology into dynamic IR drop prediction. After thorough consideration, we have decided to omit this content from the discussion and add a brief comparison of \cite{static-irdrop} in the introduction section to prevent any potential confusion between our approach and previous methodologies.


\item[R3C5]
\textbf{
Baseline model comparisons: Are the baseline models you compare PDNNet against in the results section sufficiently trained? Section IV A states that ALL the baseline models are trained using specific beta and learning rate values with a specific weight decay. However, each baseline model could need a different learning rate, etc. Is each of the baseline models sufficiently trained?
}

\item[R3A5]
% Thank you for the comment. To demonstrate each method has reached the convergence, we present the training loss curve of MAVIREC and PDNNet in the below figure. The curves all become flat as the training epochs increase. However, we could not find any training details, such as learning rate and training epochs, in \citep{chhabria_mavirec_2021}. For a fair comparison, we use the same specific training coefficient to train all the baseline models without the disturbance of different hyperparameter.

Thank you for your comment. To demonstrate the convergence of each method, we present the training loss curves for PowerNet, MAVIREC, and PDNNet in the figure below. These curves plateau as the number of training epochs increases, indicating that both methods have reached convergence. 
%
% However, we note a lack of detailed training parameters, such as learning rates and the number of epochs, in the referenced work \citep{chhabria_mavirec_2021}. 
However, we could not find any training details, such as learning rate and training epochs, in the referenced work \citep{xie_powernet_2020}  and \citep{chhabria_mavirec_2021}. 
%
%
% To ensure a fair comparison across all baseline models, we standardized the training by employing identical training coefficients. This approach mitigates the influence of varying hyperparameters, thus maintaining uniformity in our comparative analysis.
%
To ensure a fair comparison across all baseline models, we employ identical training coefficients to train all the baseline models without the disturbance of different hyperparameters.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/loss}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\item[R3C6]
\textbf{
Benchmarks: In general, the area of ML-based IR drop analysis has been very well studied in the past 5 years.  Advances in this field require significant evaluation on standard benchmark and standard metrics and comparison against prior results on the same benchmarks (to eliminate the question of ensuring the baseline models have been sufficiently trained). The recent ICCAD 2023 Problem C  had a few standard benchmarks released with standard metrics, and the results are available to the public. In fact, the contest encouraged the use of both GNNs and CNNs as the authors have done in this paper.  Can the authors add comparisons to the ICCAD Contest results using the ICCAD Contest benchmarks?
https://github.com/ASU-VDA-Lab/ML-for-IR-drop/ 
The reviewer understands that the contest was for static IR drop, and the authors are solving dynamic IR drop problem, which is more challenging. However, the authors could try training their model with the ICCAD Contest C dataset to see if their results are better than the contest. That would be helpful to ensure that we are advancing research in the ML for IR drop prediction space. It is okay if the model does not do better on static IR drop compared to ICCAD Contest results; it would still be an interesting result to show in the paper.  The use of CircuitNet is good. However, the comparisons could be made more thorough if the paper compares again prior RESULTS from the contest directly.
}

\item[R3A6]
Thank you for the comment. We conduct experiments on the ICCAD2023 contest benchmark with minimal model modification. However, we do not have good results as we only get 0.1 in F1 score and 6e-3 in MAE.
%
It seems our PDNNet does not perform well on static IR-drop prediction as our main target is just for dynamic IR-drop prediction.
%
However, designing an accurate yet effective static IR drop prediction model would be our future work.

\item[R3C7]
\textbf{
Metrics: In the case of IR drop analysis, identifying hotspots is important. In this context, several prior art, including MAVIREC, evaluate using a specific threshold and report metrics such as F1 score, false positives, false negatives, etc. How well does the PDNNet predict IR drop in regions with high IR drop? This is an important metric to show. Perhaps including numbers of F1 scores, etc., will be helpful.
}


\item[R3A7]
Thank you for the suggestion. We evaluate the F1 score value with a threshold of $90\%$ supply voltage. The results are 0.198 and 0.241 for MAVIREC and PDNNet respectively.
%
While PDNNet's F1 score surpasses that of MAVIREC, there remains potential for enhancement of our method which would be the focus of our future work.


\end{description}
\twocolumn
}



==> Doc/answer2.tex <==
{
\onecolumn
\normalsize

\ \\
\textbf{Responses to the reviewers}


We would like to firstly thank all the reviewers for their comments and our responses are as follows.

\ \\
\textbf{Reviewer 1}
\begin{description}\itemsep.8em

\item[R1C1]
\textbf{
However, the reviewer is still not fully convinced by the core graph methodology, and the current writing is still not sufficiently clear for follow-up researchers to replicate this work. For example, in the response, the author now explained that each node corresponds to a grid, and each design is divided into 256 * 256 grids. (1) Does it mean the area of each grid for different designs can be (largely) different? If yes, this will be extremely unreasonable, considering the feature is the sum of power within each grid/node. (2) Will the same feature represent different power densities when grid size differs? (3) Then how does the model transfer across designs in this case? (4) In addition, what about the layout with different heights and widths?
}


\item[R1A1]
Thank you for your valuable suggestion.
%
We address this issue by making slight adjustments to the PDNGraph generation and the PDNNet architecture. 
%
Specifically, we utilize fixed grids size \(d^x \times d^y \) to segment the layout $W \times H$, with different layout sizes corresponding to varying numbers of grids $N_w \times N_h $, $N_w = \frac{W}{d^x}$ and $N_h = \frac{H}{d^y}$, as shown in (Figure 1 (a)(b)). 
%
Each grid \( g \) is treated as a node \( v \) in our PDNGraph, ensuring a relatively uniform cell count within each node. In other words, the information represented by each node (\emph{e.g.}, power density) remains relatively consistent.
%
Thereafter, we addressed the issues of (1) and (2) raised by the reviewer through this adjustment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/multi_size_graph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%
We also slightly modify the PDNNet architecture to extract features from the updated PDNGraph, as shown in Figure 2. 
%
The graph neural network branch now performs aggregation and information propagation for PDNGraphs with varying layout with different node number $N_w \times N_h $, which reasonably capturing different PDN configuration to analyze the relationship between dynamic power consumption and IR drop. 
%
Additionally, limited by operations like downsampling in the convolutional neural network branch, direct processing of image features mapped from PDNGraph is not feasible. 
%
We align features from different layouts to fixed dimensions $H_f \times W_f\times T\times C$ that suitable for multi-scale convolution networks of CNN banch. 
%
Subsequently, the two features are concatenate by interpolation and feed to fusion module to export the predicted IR drop map. This allows our improved PDNNet to be applicable to layouts of various sizes.
%
To this end, we addressed the issues of (3) and (4) raised by the reviewer through this architecture improvement.


Note that our modified network outputs an IR drop map consistent in dimensions with the layout, enhancing its validity. For a fair comparison, we retrained all baseline methods, resulting in values that differ from those previously reported.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/pdngraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\item[R1C2]
\textbf{
The current description of the implementation of current/edge direction (a key contribution) is still very insufficient. (1) How does "PDNGraph" employ variable edge directions between nodes? (2) How does it capture the impact of (regular or irregular mesh) with the fixed 256 * 256 grids/nodes? (3) What if a grid covers a power mesh? Crisscrossed mesh? The current visualization only shows an ideal case when grids and meshes align perfectly well. (4) How is the "edge direction" in the graph formally defined? (5) The authors mentioned "... no explicit current direction between vertical nodes, we consider them as undirectional edges," but why Fig. 5 still shows vertical arrows? (6) How do the GNNs handle the graph with both directed and undirected edges?

}

\item[R1A2]
We add an algorithmic diagram (Algorithm 1) to formally illustrate the construction details of PDNGraph. 
%
The direction of the edges in PDNGraph primarily relies on our assumptions regarding the flow direction of current in the PDN. In the Figure 3, we present a example that obtains the voltage differences in both horizontal and vertical directions within a local area using the IR drop map. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/current_direction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/pdn_and_cell_revise}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Typically, current flows from high voltage area $V_{high}$ to low voltage area $V_{low}$.
%
We assume all cell share the same voltage supply $V_{supply}$ on whole layout and the voltage here is $V=V_{supply}-IR$.
%
In other words, current flows from lower IR drop areas $IR_{low}$ to higher IR drop areas $IR_{high}$ which demonstrate the IR drop map can be utilized to acquire current direction.
%

In the horizontal axis, the direction of the current edges derived from Algorithmic 1 lines 11-19, showing similarity to the direction of the IR drop differences (current map) in Figure 3 (b)(d). The average similarity score $R^2$ of 
We also calculate the similarity score $R^2$ between of IR drop differences map and our designate current edges map on dataset.
%
The score in horizontal axis is 0.2, validating the correctness of our assumptions that the current in the horizontal direction has a positional relationship with the PDN structure. 
%

Conversely, in the vertical direction, the PDN current direction has a lower similarity to the voltage drop differences (current map) in Figure 3 (c)(e).
%
The scores of all samples are less than zero, which aligns with our hypothesis that there is no significant current flow in the vertical direction (we consider it as bidirectional edges, according to lines 20-22).
%
Note that the edge directions just approximate the current directions. It does not matter that much when the real current directions differ from the edge directions we set, since we allow current values to be negative according to what is learnt from the training data. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{algorithm/pdngraph_review}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Based on the above inferences, we hereby address the reviewers' questions: 

%%%
1) As illustrated in lines 4-10 of Algorithm 1, PDNGraph primarily utilizes the smallest coordinate subtraction $s$ between set of vertical PDN's position $\{PDN^{x}\}$ in $x$ axis, and current node position $v_{i,j}^{x}$.
%
We categorize the construction of graph edges into three cases based on $s$, as illustrate in Figure 4(a)(b) corresponds to lines 12-13，Figure 4 (c) corresponds to lines 14-15, Figure 4 (d) corresponds to lines 16-17, and finally, vertical edge is determined as bidirectional corresponds to lines 20-22 in the Algorithm 1.


%%%
2) We updated PDNGraph generation process. Currently, PDNGraph can now be applied to layouts of varying sizes as well as regular and irregular PDN network structures. 

%%%
3) We illustrate the case in Figure 4 (b) where the node $v_{i,j}$ covers a PDN. In this case, $s$ is zero, which corresponds to lines 12-13 in our algorithm.

%%%
4) We formally define the "edge direction" calculate process in Algorithm 1. The details of "edge direction" are described in lines 11-22.

%%%
5) We apologize for ambiguity caused by the arrows in the diagram. The blue arrows actually indicate the direction of current flowing from the cell to GND. We have made modifications to the diagram. 

%%%
6) We apologize for the incorrect description in the paper. The undirected edges are intended to represent bidirectional edges. We have made corrections in the manuscript.





\item[R1C3]
\textbf{
Moreover, if both GNN and CNN are on grids (nodes) with the same features, and the nodes are connected in a regular graph (each node always connects to its four neighbors, left, right, up, down), GNN is turned into a spatial convolution method, which is very similar to a CNN convolution. What is the unique contribution of using GNN? Is it the direction? Please provide some insights if possible.
}

\item[R1A3]

Based on the network modifications described earlier, the GNN and CNN branches now utilize the same features, albeit of different sizes. 
%
Although both branches appear to process information similarly, as you said, the primary difference is that the graph aggregation process can select which neighbor node features to aggregate based on the directional attributes of the edges. 
%
We illustrate aggregation of directed graph and convolution process in 4 direction (top, bottom, left, right) in Figure 5 (a)(b).
%
% First, the information propagation mechanism in the graph neural network aggregates neighbor features before multiplying by node weights. In contrast, the convolutional neural network aggregates by multiplying each pixel within the convolutional range by weights before summation.
%
% As you noted, the GNN pays attention to edge direction during aggregation, with nodes only aggregating features from directed neighbor nodes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/split_conv}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Clearly, the assumptions regarding current direction in the graph will not be perceived by the CNN convolutional kernels.
%
To demonstrate the impact of these directed edges on information aggregation, we conduct an extra experiment to show that this directional information cannot be perceived by CNNs. We replace the GNN branch in PDNNet with a CNN branch designed for spatial awareness, which consists of two convolutional layers. 
%
Since conventional convolutional kernels (\emph{e.g.} \( 3 \times 3, 5 \times 5 \)) cannot aggregate information from just the four immediate neighbors (top, bottom, left, right), we employ a \( 3 \times 1\) kernel and a \( 1 \times 3\) kernel to aggregate features from horizontal and vertical neighbors (Figure 5 (c)), respectively. 
%
Our experimental results shows in Table 1, indicate that this model's performance is inferior to that of our GNN branch, demonstrating the significant role of edge direction information in enhancing aggregation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/revise2/split_conv}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\item[R1C4]
\textbf{
Some additional minor comments:
(1) What is the definition and dimension of $v_k$? 
(2) Are temporal powers used in input features?
(3) The graph is actually a regular graph (256 * 256), but the figure 3 shows an irregular graph, which is slightly misleading.
(4) The correlation improvement over MAVIREC in the shown figures is indeed not very significant.
(5) The authors may show some ground-truth patterns and indicate their correlation to current directions across power mesh. This may give great insights.
}

\item[R1A4]
Thank you for the comment. 

%%%
1)You must be referring to a symbol in the formula for feature aggregation in the GNN branch of PDNNet. We denote a specific neighbor node \( k\) within the neighborhood \( N_v \) of node  \( v\), where  \( v_k^{(l-1)} \)  represents the feature of node \( k\) at layer \( l-1\) . We add an explanation of this symbol's meaning in the methods section.

%%%
2)
Yes, our input features include the time-varying power feature \( \text{power}_t \) to predict dynamic voltage drop. Our input features consist of several power-related feature: leakage power \( \text{power}_l \) , static power \( \text{power}_s \) , switching power \( \text{power}_{sca} \) , total power \( \text{power}_{all} \) , and time-varying dynamic power \( \text{power}_t \). The dynamic power in the dataset includes instantaneous power measurements at 20 different timestamps in a time span. We use these 20 time-varying dynamic power values, along with the previous four power features, as our input features.

%%%
3)
We apologize for any misunderstanding caused by this image. Our intention was simply to indicate that we generated a graph, distinguishing it from the image features used in previous methods. We adopt your advise and update the figure in the paper accordingly.

%%%
4)
Thank you for your suggestion. We have updated the original image and chosen a better method for visualization.

%%%
5)
Current commercial power analysis tools lack the functionality to display current direction within power distribution networks. However, we adopt an alternative approach to illustrate the relationship between current direction and the PDN structure. 
%
Typically, current flows from high voltage area $V_{high}$ to low voltage area $V_{low}$.
%
We assume all cell share the same voltage supply $V_{supply}$ on whole layout and the voltage here is $V=V_{supply}-IR$.
%
In other words, current flows from lower IR drop areas $IR_{low}$ to higher IR drop areas $IR_{high}$ which demonstrate the IR drop map can be utilized to acquire current direction.
%

In the horizontal axis, the direction of the current edges derived from Algorithmic 1 lines 11-19, showing similarity to the direction of the IR drop differences (current map) in Figure 6 (b)(d). The average similarity score $R^2$ of 
We also calculate the similarity score $R^2$ between of IR drop differences map and our designate current edges map on dataset.
%
The score in horizontal axis is 0.2, validating the correctness of our assumptions that the current in the horizontal direction has a positional relationship with the PDN structure. 
%

Conversely, in the vertical direction, the PDN current direction has a lower similarity to the voltage drop differences (current map) in Figure 6 (c)(e).
%
The scores of all samples are less than zero, which aligns with our hypothesis that there is no significant current flow in the vertical direction (we consider it as bidirectional edges, according to lines 20-22).
%
Note that the edge directions just approximate the current directions. It does not matter that much when the real current directions differ from the edge directions we set, since we allow current values to be negative according to what is learnt from the training data. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/current_direction_2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 It can be observed that in the vertical direction, the computed current direction closely resembles the assumed current direction in the PDNGraph. In contrast, it is more challenging to identify the relationship between current direction and the PDN structure in the horizontal direction. This aligns with our assumption that current flows as bidirectional edges in the horizontal direction of the PDNGraph. This association between current direction and PDN structure reinforces the rationale behind our design of a PDNGraph with directed edges.

\end{description}


\ \\
\textbf{Reviewer 2}
\begin{description}\itemsep.8em


\item[R2C1]
\textbf{
I noticed that [3] captures PDN topology as an image. Are there possible comparisons between image-based PDN capturing and graph-based PDN modeling approaches?
}

\item[R2A1]
Thank you for your valuable suggestion. 
%
We compare the image-based PDN capturing and graph-based PDN in \cref{sec:method:discussion}:

%%%
A previous work \citep{static-irdrop} on static IR drop prediction also highlighted the importance of PDN structures in achieving IR drop predictions. The authors transformed the PDN structure into a PDN density map (each pixel denotes the total number of PDN strips covering this location) and an effective distance map from the power supply pins. Then, a fully convolutional network, IREDGe, utilizing these additional features for IR drop map generation. 
%
In contrast, our paradigm manifests an obvious difference with this work. 
%
Firstly, PDNGraph represents the PDN structure using a directed graph. We take into account the specific locations of the PDN on the layout and bridge finely cell-PDN physical relation during the graph construction. In cases where the PDN of a chip is relatively uniform, the PDN density map would become a uniform map which powerless to capture the PDN configuration. 
%
Secondly, the edges direction in PDNGraph simulating the current flow from the PDN structure to the cells. The graph branch in PDNNet can favorably perceive and directionally aggregate the features of neighboring features, which cannot be achieved by CNNs.

%%%
Additionally, we include the comparsion between two different PDN perception methods in the Table 2.
%
We incorporate PDN density map and power pad effective distance map in IREDGe\citep{static-irdrop} as additional features into the MAVIREC network. The results in Table 2 demonstrate that PDNNet, utilizing GNN for PDN structure perception, outperforms image-based methods. The feature extraction process of GNNs for PDN structures can be viewed as a learnable representation, offering superior expressiveness compared to fixed image-based features.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/revise2/more_feaure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\item[R2C2]
\textbf{
The figure sent in the response document regarding the training of PowerNet, Mavirec, and PDNNet, (1) I cannot see the blue curve. (2) It looks like the MAVIREC loss is also increasing. Its a concern if the models are sufficiently trained.  This is also pointed out by Reviewer 2.
}

\item[R2A2]
1) We apologize for the previous figure, where the overlapping lines of MAVIREC and PDNNet resulted in the blue lines being obscured. We separate the images to better illustrate the convergence curves in Figure 7 (a)(b).

%%%
2) We assume you refer that the loss of MAVIREC continues to decrease. We train the MAVIREC network for 600 epochs, and the convergence curve of its loss is present in Figure 8. We utilized the this MAVIREC results in our experiments.


Note that our modified network outputs an IR drop map consistent in dimensions with the layout, enhancing its validity. For a fair comparison, we retrained all baseline methods, resulting in values that differ from those previously reported.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/loss_compare}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/loss_mavi_600}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{description}

\ \\
\textbf{Reviewer 3}
\begin{description}\itemsep.8em


\item[R3C1]
\textbf{
Are the 3 IR drop maps in Fig. 7 on the same color scale? The MAVIREC seems to be biased by some extreme values.
}


%%%
\item[R3A1]
We examine the previously visualized images and found they were not on the same color scale. We update the visualizations to ensure that all images are presented on a consistent scale.


%%%
\item[R3C2]
\textbf{
In R3A4, you omitted the contents of work [3]. It makes sense in terms of the background, but I think it will be helpful to discuss the methods in [3]. [3] adopts an effective distance map to measure the distance from an instance to the power pads. There is a similarity between the effective distance map and your PDNGraph. In [3], the distance is represented by values of pixels, whereas in your work, the distance determines the current direction. The comparison between the 2 types of feature representation would be helpful to demonstrate the strength of your work, e.g. the direction of graph message passing cannot be achieved by CNNs in [3].
}


%%%
\item[R3A2]
Thank you for your valuable suggestion. 
%
We compare the image-based PDN capturing and graph-based PDN in \cref{sec:method:discussion}:

%%%
A previous work \citep{static-irdrop} on static IR drop prediction also highlighted the importance of PDN structures in achieving IR drop predictions. The authors transformed the PDN structure into a PDN density map (each pixel denotes the total number of PDN strips covering this location) and an effective distance map from the power supply pins. Then, a fully convolutional network, IREDGe, utilizing these additional features for IR drop map generation. 
%
In contrast, our paradigm manifests an obvious difference with this work. 
%
Firstly, PDNGraph represents the PDN structure using a directed graph. We take into account the specific locations of the PDN on the layout and bridge finely cell-PDN physical relation during the graph construction. In cases where the PDN of a chip is relatively uniform, the PDN density map would become a uniform map which powerless to capture the PDN configuration. 
%
Secondly, the edges direction in PDNGraph simulating the current flow from the PDN structure to the cells. The graph branch in PDNNet can favorably perceive and directionally aggregate the features of neighboring features, which cannot be achieved by CNNs.

%%%
Additionally, we include the comparsion between two different PDN perception methods in the Table 3.
%
We incorporate PDN density map and power pad effective distance map in IREDGe\citep{static-irdrop} as additional features into the MAVIREC network. The results demonstrate that PDNNet, utilizing GNN for PDN structure perception, outperforms image-based methods. The feature extraction process of GNNs for PDN structures can be viewed as a learnable representation, offering superior expressiveness compared to fixed image-based features.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/revise2/more_feature_2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%
\item[R3C3]
\textbf{
 Fig. 5 illustrates the PDNGraph construction. It can be improved to better show the strength of the GNNs, which is the irregularity and long-range information. The physical structures (power rails) will draw a lot of attention. It is recommended to stress the message-passing between nodes in the figure.
}

%%%
\item[R3A3]
Thank you for your valuable feedback. We update Figure 5 and add a message aggregation and passing paradigm to represent the feature propagation on the PDNGraph.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irr-re-context-2-revise}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\item[R3C4]
\textbf{
In the experiments of TABLE V, it is recommended to discuss the number of parameters. The experimental results in TABLE V show that your model is not simply an expansion of parameters but a reasonable fusion of 2 techniques.
}



\item[R3A4]
Thank you for your valuable suggestion. We include the parameter counts for different types of networks in the experimental section and discussed them accordingly.
%
"We have the following observations. 
%
First, although CNNs dominate the IR drop prediction in previous works, we interestingly observe that our GNN branch's performance in a single branch has similarly performance compared its CNN-based counterpart, whilst with a simple PDN perception and relatively shallow layers (two GNN layers, each accompanied by one GNN block. The parameter is also less than CNN, 41.15K vs. 17.07M).
%
This phenomenon is largely due to our specifically designed PDNGraph data structure which effectively mimics current flow and fine-grained cell-PDN relation within the PDN grid.
%
In dual-branch architecture, despite the NMAE, $R^2$ and PSNR, the dual-branch CNN have similar performance compared with GNN counterpart in other metrics.However, the parameter in dual-branch CNN is far more than GNN 34.13M vs. 78.02K.
%
Second, compared to a single-branch, dual-branch architecture indeed boosts the prediction performance.
%
However, both of these variants do not outperform our heterogeneous PDNNet (0.0358/0.0336 \emph{vs.} \textbf{0.0233}, and 0.8193/0.8232 \emph{vs.} \textbf{0.9100}) with 17.1M parameters, which demonstrate the PDN configuration and dynamic current pattern representations are two complementary aspects for effective IR drop prediction."


\item[R3C5]
\textbf{
In R2C3, the mentioned R-square for MAVIREC is oddly low, given that the NMAE of MAVIREC is not bad. Please check the correctness.
}



\item[R3A5]
We retrain the MAVIREC model for 600 epochs to achieve convergence. We update the experimental table with the latest results.
%
Note that our modified network outputs an IR drop map consistent in dimensions with the layout, enhancing its validity. For a fair comparison, we retrained all baseline methods, resulting in values that differ from those previously reported.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/review/loss_mavi_600_2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\end{description}
\twocolumn
}



==> Doc/bio.tex <==
\clearpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/yzhao}}]{Yuxiang Zhao}
received the B.E. degree in optoelectronic information science and engineering from China University of Petroleum in 2019, and the M.E. degree in control engineering from Shenzhen Institutes of Advanced Technology, Chinese Academy of Sciences, in 2022.
He is currently pursuing the Ph.D. degree with the School of Integrated Circuits at Peking University. His research interests involve deep learning and applications, physical design algorithms and implementations.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/zchai}}]{Zhuomin Chai}
    received the B.S. degree in physics from Wuhan University, Wuhan, China, in 2020.
    He is currently pursuing the Ph.D. degree at Wuhan University with the School of Physics and Technology and is a visiting student at Peking University, Beijing, China. 
    His research interests include physical designs and machine learning in CAD.
  \end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/jiangxun}}]{Xun Jiang}
received the B.E. degree in Microelectronic Science and Engineering and M.S. degree in Integrated Circuit Engineering from Nanjing University, Nanjing, China, in 2019 and 2022, respectively. He is currently pursuing the Ph.D. degree in Integrated Circuit Engineering with Peking University, Beijing, China. His current research interests include physical design and machine learning in EDA. 
  \end{IEEEbiography}




\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/ylin}}]{Yibo Lin}
(M’19) received the B.S. degree in Mi-croelectronics from Shanghai Jiaotong University in 2013. 
He obtained his Ph.D. degree in Electrical and Computer Engineering from the University of Texas at Austin in 2018 advised by Prof. David Z. Pan. 
He worked as a postdoctoral researcher at the University of Texas at Austin from 2018 to 2019. 
He currently is an assistant professor in the School of Integrated Circuits at Peking University. 
His research interests include physical design, machine learning applications, and heterogeneous computing in VLSI CAD. 
He is a recipient of the Best Paper Awards at preimier EDA/CAD journals/conferences like TCAD, DAC, DATE, ISPD, etc.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/rwang}}]{Runsheng Wang}
  (S’07–M’11) received the B.S. and Ph.D. (highest honors) degrees from Peking University, Beijing, China, in 2005 and 2010, respectively. 
  From November 2008 to August 2009, he was a Visiting Scholar with Purdue University, West Lafayette, IN, USA. 
  He joined Peking University in 2010, where he is currently a Full Professor at the School of Integrated Circuits. 
  He also serves as the Associate Dean of the School of EECS. 
  He has authored/coauthored 1 book, 4 book chapters, and over 190 scientific papers, including more than 40 papers published in International Electron Devices Meeting (IEDM) and Symposium on VLSI Technology (VLSI-T). 
  He has been granted over 20 US patents and over 30 Chinese patents. His current research interests include nanoscale CMOS devices, characterization and reliability, design-technology co-optimization (DTCO) and EDA, emerging technologies and circuits for new-paradigm computing. 
  Dr. Wang was awarded the IEEE EDS Early Career Award by the IEEE Electron Device Society (EDS), National Distinguished Young Scholars by National Natural Science Foundation of China (NSFC), Natural Science Award (First Prize) by the Ministry of Education (MOE) of China, and many other awards. 
  He serves on the Editorial Board of IEEE TRANSACTIONS ON ELECTRON DEVICES and SCIENCE CHINA: Information Sciences. He has also served on the Technical Program Committee of many IEEE conferences, including IEDM, IRPS, EDTM, IPFA, etc.
  \end{IEEEbiography}
  
  

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.24in,clip,keepaspectratio]{./Photos/rhuang}}]{Ru Huang}
  (Fellow, IEEE) received the B.S.
  (Hons.) and M.S. degrees in electronic engineering
  from Southeast University, Nanjing, China, in 1991
  and 1994, respectively, and the Ph.D. degree in
  microelectronics from Peking University, Beijing,
  China, in 1997. Since 1997, she has been a Faculty
  Member with Peking University, where she
  is currently a Professor. She is also serving as the President of Southeast University, Nanjing, China since 2022.
  She has authored or coauthored 5 books, 5 book
  chapters, and more than 300 articles, including
  more than 80 articles in IEDM (35 IEDM articles
  from 2007 to 2019), VLSI Technology Symposium, IEEE EDL, and IEEE T-ED. She has delivered over 50 keynote/invited talks at conferences and seminars. 
  She holds over 200 patents including 49 U.S. patents. 
  Her research interests include nano-scaled CMOS devices, ultralow-power new devices, new devices for neuromorphic computing, emerging memory technology, and device variability/reliability. 
  Dr. Huang is an Elected Academician of Chinese Academy of Sciences and an Elected Member of IEEE Fellow and TWAS Fellow.
  \end{IEEEbiography}
  

  

  

==> Doc/cover.tex <==
{
\twocolumn[
\begin{@twocolumnfalse}

Dear Editor and Reviewers,

\ \\
Thank you very much for reviewing and editing our submission.

Enclosed is our manuscript entitled “\emph{PDNNet: PDN-Aware GNN-CNN Heterogeneous Network for Dynamic IR Drop Prediction}”. This is an original paper that has not been published anywhere else. We look forward to contributing to IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD). Thank you in advance for your efforts on reviewing and editing.


\ \\
Best regards,
\ \\

Yuxiang Zhao

\end{@twocolumnfalse}
]
}


==> Doc/figure_table.tex <==
{
\onecolumn
\normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irdrop-vis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/method-compare} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irdrop-analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/pipeline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/pdngraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/pdn_and_cell}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{algorithm/pdngraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/irr-re-context-2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/arch}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/statistics} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/circuitnet} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Figure/visual}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/ablation1} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Tables/ablation2} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\twocolumn
}


==> Figure/distribution.tex <==

\begin{figure}[!t]
    % \vspace{-4em}
    \begin{center}
    \setlength{\tabcolsep}{1.5pt}
    \scalebox{0.97}{
    \begin{tabular}[b]{c c c c}
    
    \put(-6,-65){\rotatebox{90}{\small Probability}} &
    \includegraphics[width=.210\textwidth,valign=t]{Images/distribution/distribution1.pdf} &  
    \put(-6,-65){\rotatebox{90}{\small Probability}} & 
    \includegraphics[width=.210\textwidth,valign=t]{Images/distribution/distribution2.pdf} 
    \\
    \vspace{-4mm} %added by author2
    \  &  \ \emph{zero-riscy-a} &  \ \ \   &  \ \emph{zero-riscy-b} 
    \vspace{1mm} %added by author2
    % \hspace{-2mm}
    \end{tabular}}
    \end{center}
    % \vspace*{-5mm}
    \caption{MAE distribution of two designs in test set. The mean error of total test samples is around $2\%$.
    }
    \label{fig:distribution}
    \vspace{-1.7em}
    \end{figure}
    

==> Figure/irr-re-context-2-revise.tex <==
\begin{figure}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.48\textwidth]{Images/irr-re/revise2/v1/v1.png}
    \vspace{0.3em}
    \caption*{
    Figure 9. (a) message aggregation and passing on PDNGraph. (b) PDNGraph construction of regular PDN grid. (c) PDNGraph construction of irregular PDN grid. Generally, standard cells that are further away from the PDN experience higher IR drop.}
    % \vspace{-1.em}
    % \label{fig:irr-re}
\end{figure}


==> Figure/irr-re-context.tex <==
\begin{figure}[!h]
    % \vspace{-4em}
    \begin{center}
    \setlength{\tabcolsep}{1.5pt}
    \scalebox{0.97}{
    \begin{tabular}[b]{c}
    
    \includegraphics[width=.46\textwidth,valign=t]{Images/irr-re/v1/regular.png} 
    \\
    \vspace{4mm} %added by author2
    (a) regular mesh 
    \\
    \includegraphics[width=.45\textwidth,valign=t]{Images/irr-re/v1/irregular.png} 
    \\ (b) irregular mesh
    \vspace{1mm} %added by author2
    % \hspace{-2mm}
    \end{tabular}}
    \end{center}
    % \vspace*{-5mm}
    \caption{PDNGraph construction manner of regular and irregular PDN mesh.
    }
    \vspace{1.7em}
    \label{fig:irr-re}
\end{figure}
    

==> Figure/irr-re.tex <==

\begin{figure*}[h]
    % \vspace{-4em}
    \begin{center}
    \setlength{\tabcolsep}{1.5pt}
    \scalebox{0.97}{
    \begin{tabular}[b]{c c}
    
    \includegraphics[width=.40\textwidth,valign=t]{Images/irr-re/v1/regular.png} 
  &  
    \includegraphics[width=.38\textwidth,valign=t]{Images/irr-re/v1/irregular.png} 
    \\
    \vspace{4mm} %added by author2
    \  regular mesh  &   irregular mesh
    \vspace{1mm} %added by author2
    % \hspace{-2mm}
    \end{tabular}}
    \end{center}
    % \vspace*{-5mm}
    \caption*{IR drop difference between regular and irregular PDN mesh.
    }
    \vspace{1.7em}
    \end{figure*}
    

==> Figure/irr.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.4\textwidth]{Images/irr-re/v1/irregular.png}
    \vspace{0.3em}
    \caption*{IR drop in irregular PDN mesh.}
    % \vspace{-1.em}
\end{figure*}


==> Figure/loss.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.5\textwidth]{Images/loss/merge2.png}
    \vspace{0.3em}
    \caption*{Training loss curve of MAVIREC~\citep{chhabria_mavirec_2021}.}
    % \vspace{-1.em}
\end{figure*}


==> Figure/mavi_loss.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.5\textwidth]{Images/loss/mavi_loss.png}
    \vspace{0.3em}
    \caption*{Training loss curve of MAVIREC~\citep{chhabria_mavirec_2021}.}
    % \vspace{-1.em}
\end{figure*}


==> Figure/nmae_hist.tex <==
\begin{figure}[t]
% \vspace{-4em}
    \centering
    \includegraphics[width= 0.5\textwidth]{Images/experiment/NMAE.png}\vspace{-0.2em}
    \caption{NMAE histgram}
    \label{fig:pdngraph}
    \vspace{-1.em}
\end{figure}


==> Figure/pdngraph-head.tex <==
\begin{figure}[t]
% \vspace{1cm}
    \centering
    \includegraphics[width=0.45\textwidth]{Images/pdngraph-head/pdngraph-head-v2.pdf}
    \caption{The outline of our PDNGraph. }
    \label{fig:pdngraph-head}
    \vspace{-1.8em}
\end{figure}

==> Figure/review/current_direction.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.78\textwidth]{Images/review/current_direction/v4.png}
    \vspace{0.3em}
    \caption*{Figure 3. (a) IR drop map. (b) The horizontal current direction as defined in our PDNGraph, with red representing leftward current and blue representing rightward. (c) Vertical voltage difference, where red indicates upward current direction and blue indicates downward.    (d) Horizontal voltage difference, where red indicates leftward current direction and blue indicates rightward. (e) The vertical current direction as defined in our PDNGraph, with red representing upward current and blue representing downward.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/current_direction_2.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.78\textwidth]{Images/review/current_direction/v4.png}
    \vspace{0.3em}
    \caption*{Figure 6. (a) IR drop map. (b) The horizontal current direction as defined in our PDNGraph, with red representing leftward current and blue representing rightward. (c) Vertical voltage difference, where red indicates upward current direction and blue indicates downward.    (d) Horizontal voltage difference, where red indicates leftward current direction and blue indicates rightward. (e) The vertical current direction as defined in our PDNGraph, with red representing upward current and blue representing downward.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/loss_compare.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.85\textwidth]{Images/loss/revise2/total_compare_loss_v1.png}
    \vspace{0.3em}
    \caption*{Figure 7. Training loss curve of PDNNet, PowerNet and MAVIREC.}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/loss_mavi_600.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.6\textwidth]{Images/loss/revise2/mavi_600_v1.png}
    \vspace{0.3em}
    \caption*{Figure 8. Training loss curve of MAVIREC under 600 epochs.}
    % \vspace{-1.em}
\end{figure*}

==> Figure/review/loss_mavi_600_2.tex <==
\begin{figure*}[h]
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.6\textwidth]{Images/loss/revise2/mavi_600_v1.png}
    \vspace{0.3em}
    \caption*{Figure 10. Training loss curve of MAVIREC under 600 epochs.}
    % \vspace{-1.em}
\end{figure*}

==> Figure/review/multi_size_graph.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.58\textwidth]{Images/review/multi_size_graph/v1.png}
    \vspace{0.3em}
    \caption*{Figure 1. Layout partition diagram. (a) The layout is divided using same grid size \(d^x \times d^y \). (b) The number of PDNGraph nodes $N_w \times N_h $ adapts to the size of the layout.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/pdn_and_cell_revise.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.88\textwidth]{Images/review/pdn_and_cell/v2.png}
    \vspace{0.3em}
    \caption*{Figure 4. The figure shows how the directions of edges between nodes in PDNGraph are determined. We categorize the relationship between the nearest PDN location and the current node into four cases.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/pdngraph.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.9\textwidth]{Images/arch/revise2/v2.png}
    \vspace{0.3em}
    \caption*{Figure 2. Revised PDNNet architecture. We apply an alignment method to scale the features of the PDNGraph, which adapts to the layout size, to a fixed size  $H_f \times W_f\times T\times C$ so that they can be processed by the subsequent CNN convolution branch. Since the CNN branch mainly focuses on extracting dynamic power features, the spatial scaling has a minimal impact on the network's overall performance. The GNN and CNN features are then combined through interpolate concatenate and feed to fusion module to generate the predicted IR drop map.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/review/split_conv.tex <==
\begin{figure*}[h]
\label{fig:split_conv}
% \vspace{-1em}
    \centering
    \includegraphics[width= 0.78\textwidth]{Images/review/split_conv/v2.png}
    \vspace{0.3em}
    \caption*{Figure 5. (a) GNN aggregates information from neighboring nodes with directed edge. (b) CNN performs aggregation in the up, down, left, and right directions. (c) We use \( 1 \times 3\)  kernel and a  \( 3 \times 1\) kernel to implement CNN aggregation of the features from the four neighboring nodes for comparison experiments with GNN.}
    % \label{fig:pdngraph}
    % \vspace{-1.em}
\end{figure*}


==> Figure/speed-acc.tex <==
\begin{figure}[!t]
% \vspace{-3em}
    \centering
    \includegraphics[width= 0.47 \textwidth]{Images/experiment/speed-accuracy-v5.pdf}
    \vspace{0.2em}
    \caption{Accuracy-computation trade-off on CircuitNet for different methods in the inference phase. The horizontal axis shows the inference cost (\emph{i.e.}, whole inference time or model inference time) per sample. Whole inference time includes data processing and model inference.}
    \label{fig:speed-acc}
    % \vspace{-1em}
\end{figure}


==> Tables/mini-circuitnet.tex <==
\begin{table*}
% \vspace{-1em}
\begin{center}
\caption{\small Evaluation results on Mini-CircuitNet dataset. 
%
\textcolor{red}{Red} denotes percentage of improvement.
%
$\downarrow$ means “lower is better”, $\uparrow$ means “higher is better”.}
\label{table:mini}
% \vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.05}{
    \centering
    \setlength{\tabcolsep}{4mm}{
    \begin{tabular}{l | c c c c c}
    \toprule[0.12em]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Mini-CircuitNet}} \\
    \cline{2-6}
         & 
        NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        PowerNet~\citep{xie_powernet_2020} & 0.171 & 0.62 & 0.75 & 0.70 &  0.60 \\ 
                
        \textbf{PDNNet} (Ours) &
         \textbf{0.034}(\textcolor{red}{-80.1\%}) & \textbf{0.87}(\textcolor{red}{+40.3\%}) & \textbf{0.94}(\textcolor{red}{+25.3\%}) & \textbf{0.75}(\textcolor{red}{+7.1\%}) & \textbf{0.62}(\textcolor{red}{+3.3\%})\\ 
         \midrule
        MAVIREC~\citep{chhabria_mavirec_2021} & 0.056 & 0.82 & 0.92 & 0.71 & 0.58 \\ 

        \textbf{PDNNet} (Ours) & \textbf{0.034}(\textcolor{red}{-39.3\%}) & \textbf{0.87}(\textcolor{red}{+6.09\%}) & \textbf{0.94}(\textcolor{red}{+2.2\%}) & \textbf{0.75}(\textcolor{red}{+5.6\%}) & \textbf{0.62}(\textcolor{red}{+6.9\%})\\ 
        \bottomrule[0.12em]
    \end{tabular}}}
\end{center}
% \vspace{-1.em}
\end{table*}


==> Tables/revise2/more_feature_2.tex <==
\begin{table*}[h]
% \vspace{-3em}
\begin{center}
\caption*{Table 3 \small The comparison between PDNNet and image-based method. We add the PDN related image features (PDN density, power pad effective distance) to MAVIREC network.}
\label{table:gnn}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \begin{tabular}{l c c c c c c c}
    \toprule[0.12em]
        Network & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        MAVIREC+image-based PDN features &0.0372  & 0.8150& 18.5548 & 0.6953 & 0.9127 &0.8585 & 0.7813
        \\ 
        \textbf{PDNNet} & 0.0282 & 0.8369 & 19.3483 & 0.7190 & 0.9186 & 0.8709 & 0.8064 \\ 
        \bottomrule[0.12em]
    \end{tabular}}
    % \vspace{-1.3em}
\end{center}
\end{table*}


==> Tables/revise2/more_feaure.tex <==
\begin{table*}[h]
% \vspace{-3em}
\begin{center}
\caption*{Table 2 \small The comparison between PDNNet and image-based method. We add the PDN related image features (PDN density, power pad effective distance) to MAVIREC network.}
\label{table:gnn}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \begin{tabular}{l c c c c c c c}
    \toprule[0.12em]
        Network & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        MAVIREC+image-based PDN features &0.0372  & 0.8150& 18.5548 & 0.6953 & 0.9127 &0.8585 & 0.7813
        \\ 
        \textbf{PDNNet} & 0.0282 & 0.8369 & 19.3483 & 0.7190 & 0.9186 & 0.8709 & 0.8064 \\ 
        \bottomrule[0.12em]
    \end{tabular}}
    % \vspace{-1.3em}
\end{center}
\end{table*}


==> Tables/revise2/split_bk.tex <==
\begin{table*}[h]
% \vspace{-3em}
\begin{center}
\caption*{Table 1 \small The comparison between the aggregation methods of GNN and CNN, our GNN demonstrates superior results in perceiving edge directions compared to CNN.}
\label{table:gnn}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \begin{tabular}{l c c c c c c c}
    \toprule[0.12em]
        Network & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        CNN Aggregation &  0.0465 & 0.8121 & 18.7550 & 0.5923 & 0.9122 & 0.7597 & 0.6232
        \\ 
        \textbf{PDNNet} & \textbf{0.0233} & \textbf{0.9100} & \textbf{21.8670} & \textbf{0.8139} & \textbf{0.9552} & \textbf{0.9231} & \textbf{0.8574} \\ 
        \bottomrule[0.12em]
    \end{tabular}}
    % \vspace{-1.3em}
\end{center}
\end{table*}


==> Tables/revise2/split_conv.tex <==
\begin{table*}[h]
% \vspace{-3em}
\begin{center}
\caption*{Table 1 \small The comparison between the aggregation methods of GNN and CNN, our PDNNet with GNN branch demonstrates superior results in perceiving edge directions compared to CNN.}
\label{table:gnn}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \begin{tabular}{l c c c c c c c}
    \toprule[0.12em]
        Network & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        CNN Spatial-Temporal Aggregation & 0.0360 & 0.8117 & 18.6830 & 0.6992 & 0.9107 & 0.7051 & 0.5750
        \\ 
        \textbf{PDNNet} & 0.0282 & 0.8369 & 19.3483 & 0.7190 & 0.9186 & 0.8709 & 0.8064 \\ 
        \bottomrule[0.12em]
    \end{tabular}}
    % \vspace{-1.3em}
\end{center}
\end{table*}


==> Tables/statics-bk.tex <==
\begin{table}[tb]
\vspace{-1em}
\begin{center}
\caption{\small The statistics of Mini-CircuitNet. Samples randomly sample from the origin superset. Note that training \& testing datasets have no intersection in designs.}
\label{table:statistics}
\vspace{1mm}
\setlength{\tabcolsep}{3.0pt}
\scalebox{0.9}{
    \centering
\begin{tabu}{l|c|c|ccc|c}
\toprule[0.12em]
\multirow{3}{*}{}      & \multirow{3}{*}{Design} & \multirow{3}{*}{\makecell{Number \\ of \\  Samples}} & \multicolumn{3}{c}{Netlist Statistics}    & \multirow{3}{*}{\makecell{IR drop \\ value \\(mV)}}      \                                                                   \\ \cline{4-6} 
                       &                &          & \multicolumn{1}{c}{\#Cells} & \multicolumn{1}{c}{\#Nets} & \begin{tabular}[c]{@{}c@{}}Cell Area\\ ($\mu m^2$)\end{tabular} & \\
                       \midrule[0.12em]
\multirow{4}{*}{Train} & \texttt{RISCY-a} & 20 & \multicolumn{1}{c}{44,836}       & \multicolumn{1}{c}{80,287}      &   65,739 & 5.43 \\
                       & \texttt{RISCY-b} & 22 & \multicolumn{1}{c}{30,207}   & \multicolumn{1}{c}{58,452}  & 69,779  & 6.28\\ 
                       & \texttt{RISCY-FPU-a} & 21 & \multicolumn{1}{c}{61,677}       & \multicolumn{1}{c}{106,429}      &  75,985  & 8.45\\ 
                       & \texttt{RISCY-FPU-b} &  17  & \multicolumn{1}{c}{47,130}   & \multicolumn{1}{c}{84,676}  & 80,030 & 8.73 \\ 
                       \midrule
\multirow{2}{*}{Test}  & \texttt{zero-riscy-a} & 13   & \multicolumn{1}{c}{35,017}   & \multicolumn{1}{c}{67,472}  & 58,631  & 4.84 \\ 
                       & \texttt{zero-riscy-b} & 7  & \multicolumn{1}{c}{20,350}   & \multicolumn{1}{c}{45,599}  & 62,648  & 4.36\\ 
    \bottomrule[0.12em]
    \end{tabu}}
\end{center}
\vspace{-2em}
\end{table}

==> Tables/visual_compare_1.tex <==
\begin{table*}[h]
% \vspace{-1em}
\begin{center}
\caption*{\small Evaluation results on visual case 1. 
%
$\downarrow$ means “lower is better”, $\uparrow$ means “higher is better”.}
\label{table:compare_1}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l | c c c c c c c}
    \toprule[0.12em]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c}{\textbf{Case1}}  \\
    \cline{2-8}
         & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$\\ 
        \midrule[0.12em]
        MAVIREC & 0.0242  & \textbf{0.9554} & 21.8843 & 0.7875 & 0.9776 & 0.8163 & 0.6796 \\ 
                
        \textbf{PDNNet} (Ours) & \textbf{0.0231} & 0.9474 & \textbf{23.2063} & \textbf{0.8361} & \textbf{0.9789} & \textbf{0.8244} & \textbf{0.7104} \\ 
        \bottomrule[0.12em]
    \end{tabular}}}
\end{center}
% \vspace{-1.em}
\end{table*}



==> Tables/visual_compare_2.tex <==
\begin{table*}[h]
% \vspace{-1em}
\begin{center}
\caption*{\small Evaluation results on visual case 2. 
%
$\downarrow$ means “lower is better”, $\uparrow$ means “higher is better”.}
\label{table:compare_2}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l | c c c c c c c}
    \toprule[0.12em]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c}{\textbf{Case 2}}  \\
    \cline{2-8}
         & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$\\ 
        \midrule[0.12em]
        MAVIREC & 0.0249  & \textbf{0.9277} & 20.0407 & 0.8349 & \textbf{0.9776} & 0.7158 & 0.5960 \\ 
                
        \textbf{PDNNet} (Ours) & \textbf{0.0201} &0.9266 & \textbf{22.3799} & \textbf{0.8630} & 0.9643 & \textbf{0.7193} & \textbf{0.5975} \\ 
        \bottomrule[0.12em]
    \end{tabular}}}
\end{center}
% \vspace{-1.em}
\end{table*}



==> Tables/visual_compare_3.tex <==
\begin{table*}[h]
% \vspace{-1em}
\begin{center}
\caption*{\small Evaluation results on visual case 3. 
%
$\downarrow$ means “lower is better”, $\uparrow$ means “higher is better”.}
\label{table:compare_3}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l | c c c c c c c}
    \toprule[0.12em]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c}{\textbf{Case 3}}  \\
    \cline{2-8}
         & NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$\\ 
        \midrule[0.12em]
        MAVIREC & 0.0349  & \textbf{0.9334} & 19.5755 & 0.7473 & \textbf{0.9675} & \textbf{0.8249} & \textbf{0.6857} \\ 
                
        \textbf{PDNNet} (Ours) & \textbf{0.0285} &0.9281 & \textbf{21.2359} & \textbf{0.7702} & 0.9662 & 0.8201 & 0.6751 \\ 
        \bottomrule[0.12em]
    \end{tabular}}}
\end{center}
% \vspace{-1.em}
\end{table*}



==> Tables/wider_network.tex <==
\begin{table*}[h]
% \vspace{-1.5em}
\begin{center}
% \caption{\small Influence of GNN \& CNN branch of PDNNet. 
% % GNN and CNN  show similar accuracy, while composed together to form the heterogeneous PDNNet present better performance.
% }
% \label{table:dual-branch}
\vspace{0.3em}
\setlength{\tabcolsep}{2.0pt}
\scalebox{1.1}{
    \centering
    \begin{tabular}{l| c c |c c c c c c c c}
    \toprule[0.12em]
        \textbf{Network} & Branch Type &  Kernel Number &    
        NMAE~$\textcolor{black}{\downarrow}$ & $R^2$~$\textcolor{black}{\uparrow}$ & 
         PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ &
         Pear~$\textcolor{black}{\uparrow}$ & Spea~$\textcolor{black}{\uparrow}$ & Kend~$\textcolor{black}{\uparrow}$ \\ 
        \midrule[0.12em]
        \multicolumn{1}{l|}{\multirow{4}{*}{CNN}} 
          & Single Branch        & $\times$ 1   & 0.0350 & 0.7728 & 20.3542 & 0.7612 & 0.9283 & 0.7434 & 0.6162 \\ 
          & Single Branch        & $\times$ 2   &0.0346 & 0.8754 & 20.4192 & 0.7647 & 0.9439 & 0.7474 & 0.6226 \\ 
          & Single Branch        & $\times$ 4  & 0.0329 & 0.8794 & 20.5947 & 0.7664 & 0.9434 & 0.7480 & 0.6236 \\ 
          & Dual Branch        & $\times$ 1  & 0.0327 & 0.8888 & 20.8586 & 0.7726 &0.9489 & 0.7462 & 0.6248 \\ 
        \midrule 
        \multicolumn{1}{l|}{\multirow{4}{*}{GNN}} 
          & Single Branch        & $\times$ 1   & 0.0315 & 0.8838 & 20.7989 & 0.7635 & 0.9427 & 0.7408& 0.6036 \\
          & Single Branch        & $\times$ 2   &0.0311 & 0.8867 & 20.9050 & 0.7636 & 0.9437 & 0.7376 & 0.6002 \\ 
          & Single Branch        & $\times$ 4  & 0.0310 & 0.8873 & 20.9234 & 0.7627 & 0.9440 & 0.7338 & 0.5964 \\ 
          & Dual Branch        & $\times$ 1  & 0.0314 & 0.8859 & 20.8536 & 0.7673 & 0.9448 & 0.7412 & 0.6042  \\ 
        \bottomrule[0.12em] 
    \end{tabular}}
\end{center}
% \vspace{-1.em}
\end{table*}


==> Textlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\iffalse
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=35pt, bottom=45pt, 
    left=40pt, right=40pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\fi
\iftrue
\geometry{twoside=true, head=13pt,
paperwidth=8.5in, paperheight=11in,
includeheadfoot, columnsep=2pc,
top=57pt, bottom=73pt, inner=54pt, outer=54pt,
marginparwidth=2pc,heightrounded
}%
\fi
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\let\Bbbk\relax % redefined in newtxmath.sty
\newcommand\hmmax{0}
\newcommand\bmmax{0}
% \usepackage{amssymb}
% \usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
%\usepackage{siunitx}
%\sisetup{product-units = single}
% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\mx}{\m{x}}
\newcommand{\my}{\m{y}}
\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}



% yuxiang setting

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{biblatex}
% \usepackage[a4paper, total={184mm,239mm}]{geometry}
% % \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
% %     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\graphicspath{{./Images/}}
\usepackage{color}
\usepackage{xcolor}
\usepackage{threeparttable}
\usepackage{utfsym}
\usepackage{url}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{subfig}
\usepackage{float}
% \usepackage{algorithm}
\usepackage{cleveref}
\usepackage{hyperref}
\usepackage[export]{adjustbox}
% \usepackage[margin = 3.5cm]{geometry}     % avoid `overfull \hbox' warning
\usepackage[tableposition = top]{caption} % captions
\usepackage{booktabs}                     % horizontal lines in tabless
\usepackage[per-mode = symbol]{siunitx}   % physical quantities and SI units
\usepackage{colortbl,booktabs}
\usepackage{multicol}
\usepackage{multirow} 
\usepackage{multirow, makecell, caption}
\usepackage{diagbox}

\usepackage{booktabs}
% \usepackage{ThreePartTable} 
\usepackage{tabu}
\usepackage{tabularx}
\usepackage{rotating}
\usepackage{supertabular}
\usepackage{tikz}
\usepackage{hhline}
\usepackage{longtable}
\usepackage{svg}
\usepackage{rotating}
\usepackage{xcolor}
\usepackage{bbding}
% \usepackage[fontsize=9pt]{fontsize}

\geometry{twoside=true, head=13pt,
paperwidth=8.5in, paperheight=11in,
includeheadfoot, columnsep=2pc,
top=30pt, bottom=50pt, inner=42pt, outer=42pt,
marginparwidth=2pc,heightrounded
}%
 % \addbibresource{./Ref/bib.bib}



==> Textlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfig}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command


\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}


% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> algorithm/pdngraph_review.tex <==

\begin{algorithm}[h]
\caption*{Algorithm. 1: PDNGraph Construction Algorithm}
\begin{algorithmic}[1]
\REQUIRE Layout dimensions $W$ and $H$, grid $g$ with fixed size ($d^x$, $d^y$), a set of vertical PDN with $x$ axis position $\{PDN^{x}\}$.
\ENSURE Our PDNGraph.

\STATE Divide the layout using grid $g$, $N_w= \frac{W}{d^x}, N_h= \frac{H}{d^y}$.

\FOR {$i = 1$ to $N_h$}
    \FOR {$j = 1$ to $N_w$}
        \STATE Set the initial value $s = \infty$.
        
        \FOR {each $PDN^{x}_{k}$ in $\{PDN^{x}\}$}
            \STATE Compute the coordinate subtraction $s$ between $PDN_{k}$ and current node $v_{i,j}$, $s\_tmp = PDN^{x}_{k} - v_{i,j}^{x}$.
            \IF {$s\_tmp < s$}
                \STATE $s = s\_tmp$
            \ENDIF
        \ENDFOR
        
        \IF {$j < N_w$}
            \IF {$s \leq 0$}
                \STATE Set the edge direction from node $v_{i,j}$ to $v_{i,j+1}$ (the closest $PDN$ is on the left of the current node $v_{i,j}$), edge is $ v_{i,j} \longrightarrow v_{i,j+1}$.
            \ELSIF {$0< s \leq 1$} 
                \STATE Set the bidirectional edge between node $v_{i,j}$ and $v_{i,j+1}$ (the closest $PDN$ is between node $v_{i,j}$ and $v_{i,j+1}$), edge is $ v_{i,j} \longleftrightarrow v_{i,j+1}$. 
            \ELSIF {$1<s$}
                \STATE Set the edge direction from node  $v_{i,j+1}$ to $v_{i,j}$ (the closest $PDN$ is on the right of the current node $v_{i,j}$ and neighbor node $v_{i,j+1}$), edge is $ v_{i,j+1} \longrightarrow v_{i,j}$.
            \ENDIF
        \ENDIF
        
        \IF {$i < N_h$}
            \STATE Set the bidirectional edge between node $v_{i,j}$ and $v_{i+1,j}$, edge is $v_{i,j} \longleftrightarrow v_{i+1,j}$.
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

